Cause-effect inference through spectral independence in linear dynamical systems: theoretical foundations

Distinguishing between cause and effect using time series observational data is a major challenge in many scientific fields. A new perspective has been provided based on the principle of Independence of Causal Mechanisms (ICM), leading to the Spectral Independence Criterion (SIC), postulating that the power spectral density (PSD) of the cause time series is uncorrelated with the squared modulus of the frequency response of the filter generating the effect. Since SIC rests on methods and assumptions in stark contrast with most causal discovery methods for time series, it raises questions regarding what theoretical grounds justify its use. In this paper, we provide answers covering several key aspects. After providing an information theoretic interpretation of SIC, we present an identifiability result that sheds light on the context for which this approach is expected to perform well. We further demonstrate the robustness of SIC to downsampling - an obstacle that can spoil Granger-based inference. Finally, an invariance perspective allows to explore the limitations of the spectral independence assumption and how to generalize it. Overall, these results support the postulate of Spectral Independence is a well grounded leading principle for causal inference based on empirical time series.

==> lemma_ident_genmodel.tex <==

Coming back to our generative model in \cref{gen_model}, it is noticable that with the increase of the order of FIR filter, $|\h_{\X\to\Y}|^2$ will be less smooth and there deviate from smoothness assumption imposed in section (ii) of proposition \ref{lem:violataion}. However we claim that in this case the randomness in selection of $\h_{\X\to\Y}$ will bound $\rho_{\Y\to\X}$ away from $1$ as a complimentary result, as the following lemma shows:
\begin{lem}\label{lem:fir_fb}
Finally if $\mathcal{L}$ is a FIR filter chosen randomly from the generative model described in \cref{gen_model}, for any given $0<\epsilon<1$ there exist $c_\epsilon > 0$ such that 
\begin{gather}
\label{FIRfbineq}
\rho_{\textbf{X}\to \textbf{Y}}.\rho_{\textbf{Y}\to \textbf{X}}\leq c_\epsilon,
\end{gather}
with probability $\delta = 1 - \exp\left(- \frac{m\pi}{4e}\right)$. Moreover $c_\epsilon$ tends to zero as $\epsilon$ approaches to zero.
\end{lem}
The proof is presented in the appendix for the sake of conciseness.
\begin{figure}

\section{Proof for \Cref{lem:fir_fb}}
The proof for \cref{lem:fir_fb} is long enough that we dedicated a section for it. To make the understanding of the proof easier, we broke down the proof into lemmas that together complete the proof. In the following section $m$ exactly represents the order of the FIR filter in section \cref{lem:fir_fb}. Additionally in this section we will use a slightly different definition of Discrete Fourier Transform from which simplifies some approximations in the proofs below significantly; previously introduced DFT would have a expression dependent on the parity of the DFT order. Moreover we will only rely on DFT of order $m$ and as result will omit mentioning the order for DFT in this section. Here we use the following definition (a slight modification of \cite[][pp. 542]{oppenheim1989discrete}) where we represent the DFT of a vector $X=(X_0, ..., X_{m-1})$ with $\tilde{X}$:
\begin{gather*}
\forall \nu=\frac{k}{m},\ k \in \left\{0, \frac{1}{m}, \frac{2}{m}..., \frac{m-1}{m}\right\},\ \ \ \tilde{X}(\nu):=\tilde{X}_{k}:=\frac{1}{\sqrt{m}}\sum\limits_{t=0}^{m-1} X_t e^{-2\pi i t\nu}.
\end{gather*}
Now assume $X$ represents a random vector, with a uniform distribution from a sphere $S^{m-1}$. One way of introducing such a random vector, beside the Haar measure, is \cite{marsaglia1972choosing} to take a random vector $X'=(X'_0,..., X'_{m-1})$ such that $X'_i \overset{i.i.d}{\sim} \mathcal{N}(0,1)$ and then define
\begin{gather}\label{eq:x_i}
X_i := \frac{X'_i}{\sum_{i=0}^{m-1} {X'_i}^2}.
\end{gather}
The coordinates of $X$ are dependent random variables (through the normalizing factor) and analyzing the behavior of a function dependent on $X$ can be hard; notice that this is the case for the generative model in \cref{lem:fir_fb}; IR function of these filters is such a random vector and $|\hat{h}(.)|^2$ is the fucntion that we are interested in statistics of it. To simplify the analysis, we rather study the behaviour of $Y=(Y_0, ..., Y_{m-1})$, which its coordinates are defined as follows:
\begin{gather}\label{eq:y_i}
Y_i = \frac{1}{\sqrt{m}} X'_i.
\end{gather}
The following lemma shows that though $Y_i$'s are independent, $Y$ can be a good representative to study the statistics of $X$.
\begin{lem}\label{lem:sphere_stats}
Take $X$ and $Y$ to be as defined in \cref{eq:x_i} and \cref{eq:y_i}. Then
$$P(\|X-Y\| < t) < 1 - 2e^{-mt^2/8}:$$
\end{lem}
\begin{proof}
{
Take $A = \left\{\omega\in\Omega \middle| \|X(\omega)-Y(\omega)\| \geq t\right\}$. Then we have:
\begin{gather}
A = \left\{\omega\in\Omega \middle| \|X(\omega)-Y(\omega)\|^2 \geq t^2\right\} = \left\{\omega\in\Omega \middle| \sum_{i=0}^{m-1} \left( X_i(\omega)-Y_i(\omega) \right)^2  \geq  t\right\} = \notag \\
\left\{\omega\in\Omega \middle| \sum_{i=0}^{m-1} \left( X_i(\omega)-Y_i(\omega) \right)^2  \geq  t\right\} = \notag \\
\left\{\omega\in\Omega \middle| \left( \frac{1}{\sum_{i=0}^{m-1} {X'_i}(\omega)^2} - \frac{1}{m} \right) \sum_{i=0}^{m-1} {X'_i}(\omega)^2  \geq  t\right\} = \notag \\
\label{eq:var_sum} \left\{\omega\in\Omega \middle| \left( 1 - \frac{\sum_{i=0}^{m-1} {X'_i}(\omega)^2}{m} \right)  \geq  t\right\}.
\end{gather}
However it is known \cite[][pp. 21]{wainwright2014high} that \cref{eq:var_sum} has indeed a low probability, .i.e. 
\[
\Pr \left(\left\{\omega\in\Omega \middle| \left( 1 - \frac{\sum_{i=0}^{m-1} {X'_i}(\omega)^2}{m} \right)  \geq  t\right\}\right) \leq 2e^{-mt^2/8}
\]
which completes the proof.
}
\end{proof}
\begin{lem}
If $X$ is an $m$-dimensional random vector where $X_i \overset{i.i.d.}{\sim}  \mathcal{N}(0,1)$ then $\tilde{X}_k|^2 \overset{i.i.d.}{\sim} \chi_2^2$ where $|\cdot|^2$ represents the absolute modulus and $\chi^2_2$ is the $\chi^2$-distribution of order $2$.
\end{lem}
\begin{proof}
See the derivation in \cite[][pp. 231-232]{jenkins1968spectral}.
\end{proof}
\begin{lem}
Suppose $f\in C^3(\mathbb{R})$ is a periodic function with period of $1$. Then:
\begin{gather*}
\left| \int^{1}_{0} f(\nu) d\nu - \frac{1}{m} \sum\limits_{i=0}^{m-1} f(\frac{k}{m}) \right| = -\frac{f''(\xi)}{12 m^2},
\end{gather*}
for some $\xi \in [0,1]$.
\end{lem}
\begin{proof}
Using Trapezoid rule for integration we get \cite{atkinson2008introduction}:
\[
\int_0^1 f(x)\,dx - \frac{1}{m} \left[ {f(0) + f(1) \over 2} + \sum_{k=1}^{m-1} f \left( \frac{k}{m} \right) \right] = -\frac{f''(\xi)}{12 m^2}.
\]
Now since $f(0)=f(1)$ the claim follows.
\end{proof}
\begin{lem}
Suppose $X_i \overset{i.i.d.}{\sim} \chi^2_2$. Then for any given $t$ and $\epsilon>0$,
\[
\frac{1}{m}\sum\limits_{i=1}^{m} \frac{1}{X_i+\epsilon} \in \left[ \frac{1}{4}\ln \left( 1 + \frac{4}{\epsilon} \right) - t, \frac{1}{2}\ln\left(1+\frac{2}{\epsilon}\right) +t \right]
\]
with probability of at least $1-2e^{-2mt^2\epsilon^2}$.
\end{lem}
\begin{proof}
{
Define $Y_i=\frac{1}{X_i+\epsilon}$. First we calculate $\E(Y)$:
\[
\E(Y)=\int_{0}^{\infty} \frac{p_{\chi^2_2}(x)}{x+\epsilon}dx.
\]
Applying the change of variable $z=(x+\epsilon)/2$ we get:
\[
\E(Y)=\frac{1}{2}\int_{\epsilon/2}^{\infty} \frac{e^{-(z-\frac{\epsilon}{2})}}{z}dz=\frac{e^{\epsilon/2}}{2}E_1(\frac{\epsilon}{2})
\]
where $E_1(x)$ is the exponential integral. Using the known bounds for exponential integral \cite{abramowitz1964handbook} we get:
\[
\frac{1}{2}\ln\left(1+\frac{4}{\epsilon}\right)< \frac{e^{\epsilon/2}}{2}E_1(\frac{\epsilon}{2}) < \ln\left( 1+\frac{2}{\epsilon}\right)
\]
Now since for all $i$ we have $Y_i\in [0,1/\epsilon]$, using Hoeffding bound we get
\[
\Pr \left( \left| \bar{Y} - \E(Y)\right|\geq t \right) \leq 2e^{-2m\epsilon^2t^2}.
\]
Therefore
\begin{gather*}
\Pr \left(\bar{Y} - \frac{1}{2}\ln \left(1 + \frac{2}{\epsilon} \right) \geq t \right)+\Pr \left( \bar{Y} - \frac{1}{4} \ln\left( 1+\frac{4}{\epsilon} \right) \leq -t \right) \leq \\ 
\Pr \left( \bar{Y} - \E(Y) \geq t \right) + \Pr \left( \bar{Y} - \E(Y) \leq - t \right) \leq 2e^{-2m\epsilon^2t^2}, 
\end{gather*}
which completes the proof.
}
\end{proof}
In \cref{lem:sphere_stats} we should that the statistical properties of $X$ and $Y$ (as defined for \cref{lem:sphere_stats}) are similar. Next argument shows that this is even true even if we apply the continuous function $h$ defined below, to both of these vectors.
\begin{lem}
Suppose for a given $\epsilon>0$,  $h: S^{m-1}\to \mathbb{R}$ is defined as below:
\[
\forall Z\in S^{m-1}(\mathbb{R}),\ h(Z) := \frac{1}{m} \sum_{i=0}^{m} \frac{1}{Z_i + \epsilon}.
\]
Then for random vectors $X$ and $Y$ as defined for \cref{lem:sphere_stats} we get:
$$\Pr(|h(X)-h(Y)|>t)<e^{-\frac{m^2t^2}{\epsilon^2}}$$
\end{lem}
\begin{proof}
\naji{I was too hopeless to complete this one but it follows by using multidimensional mean value theorem for $h$.}
\end{proof}
%\begin{proof}
%{
%Take ${\bf b}$, ${\bf h}$ and $U$ to be as defined in \cref{gen_model}. First we show that an inequality like (\ref{FIRfbineq}) would hold if we approximate $\widehat{{\bf h}}$ with a DFT of order $m$ applied to ${\bf b}$ and we represent it with $\widehat{{\bf b}}:=(\hat{b}_1, ..., \hat{b}_m)$. Accordingly assume $\rho'_{\X \to \Y}$ and $\rho'_{\Y \to \X}$ are the counterparts of original SDRs in this simplified discrete Fourier transform form of the problem. Assume that $\widehat{\bf h}(\nu)$, the transfer function of the FIR filter, is defined on $[0,1)$ domain (rather than $[-1/2, 1/2)$). Due to Parseval's theorem we have:
%$$\sum_{i=1}^{m} |\widehat{b}_i|^2=\|{\bf b}\|^2 \overset{(*)}{=} 1,$$
%where $(*)$ is assumed without loss of generality, by normalizing the energy of the filter. Notice that this means we can rephrase the generating model in terms of applying a rotation matrix $U$ to $|{\bf \widehat{b}}|$. To conclude that $\int |\hat{h}(\nu)|^{-2} d\nu$ can be large (and consequently $\rho_{\X \to \Y} \rho _{\Y \to \X}$ to be small) with high probability, it would be sufficient to show that $\eta$ defined as
%$$\eta := \sum_{i=0}^{m-1} |\widehat{b}^U_i|^2 \sum_{i=0}^{m-1} \frac{1}{|\widehat{b}^U_i|^2} = \sum_{i=0}^{m-1} \frac{1}{|\widehat{b}^U_i|^2},$$
%since 
%$$\eta\leq \int \frac{1}{|\hat{h}(\nu)||^{2}} d\nu.$$
%Now notice that $U|{\bf b}|$ is uniformly sampled from $S^m$, where $S^m$ is the $m$-dimensional centered sphere. Therefore the problem can be rephrased \cite{marsaglia1972choosing} as sampling $(X_1, X_2, ..., X_m)/\sqrt{X_1^2 + ... + X_m^2}$, where $X_i \sim \mathcal{N}(0,1)$.
%We claim that we can equivalently study the statistical properties of 
%$$ \sum_{i=1}^{m} \frac{m}{X_i^2},$$
%where $X_i \sim \mathcal{N}(0,1)$. Define 
%$$Y_i^2 :=\frac{1}{ X_i^2 + \epsilon} {\rm\ \ and\ }\ \bar{Y} := \frac{1}{m} \sum_{i=1}^{m} Y_i^2.$$
%Based on \cref{lem:approx} for $\epsilon<1$ we have:
%\begin{gather}
%\label{eq:exp_bounds}
%\E_{X_i}(Y_i) \in \left[\sqrt{\frac{\pi}{2 e}}\frac{1}{2\sqrt{\epsilon}}, \frac{1}{\epsilon}\right].
%\end{gather}
%Using Hoeffding's \cite[Theorem 2]{hoeffding1963probability} inequality for bounded random variables and \cref{eq:exp_bounds} we get:
%$$\Pr \left( \bar Y \leq \sqrt{\frac{\pi}{2 e}} \frac{1}{4\sqrt{\epsilon}} \right) \leq \Pr \left(\E(\bar Y) - \bar Y \geq  \sqrt{\frac{\pi}{2 e}} \frac{1}{4\sqrt{\epsilon}}  \right)\leq \exp\left(- \frac{m\pi}{4e} \right)$$
%and therefore
%\[
%\Pr \left( \eta \geq \sqrt{\frac{\pi}{2 e}} \frac{1}{4\sqrt{\epsilon}} \right) \geq \Pr \left( \bar Y \geq\sqrt{\frac{\pi}{2 e}} \frac{1}{4\sqrt{\epsilon}} \right) \geq 1 - \exp\left(- \frac{m\pi}{4e} \right)
%\]
%Taking 
%$$c_\epsilon = \sqrt{\frac{2 e}{\pi}} \frac{4}{m} \sqrt{\epsilon}$$
%completes the proof.
%}
%\end{proof}
